Parameterized Differential Dynamic Programming

Differential Dynamic Programming (DDP) is an efficient trajectory optimization algorithm relying on second-order approximations of a system's dynamics and cost function, and has recently been applied to optimize systems with time-invariant parameters. Prior works include system parameter estimation and identifying the optimal switching time between modes of hybrid dynamical systems. This paper generalizes previous work by proposing a general parameterized optimal control objective and deriving a parametric version of DDP, titled Parameterized Differential Dynamic Programming (PDDP). A rigorous convergence analysis of the algorithm is provided, and PDDP is shown to converge to a minimum of the cost regardless of initialization. The effects of varying the optimization to more effectively escape local minima are analyzed. Experiments are presented applying PDDP on multiple robotics systems to solve model predictive control (MPC) and moving horizon estimation (MHE) tasks simultaneously. Finally, PDDP is used to determine the optimal transition point between flight regimes of a complex urban air mobility (UAM) class vehicle exhibiting multiple phases of flight.

==> sections/ddp.tex <==
\section{Differential Dynamic Programming}

We consider discrete-time dynamics that evolve according to
\begin{align}
    \mathbf{x}_{t + 1} = \mathbf{F}(\mathbf{x}_t, \mathbf{u}_t) \label{eq/dynamics}
,\end{align}
where $\mathbf{x}_t \in \R^{n_x}$ is the state and $\mathbf{u}_t \in \R^{n_u}$ is the control.

Defining the control sequence as $\mathbf{U} \defeq \{\mathbf{u}_1, \ldots, \mathbf{u}_T\}$, the discrete-time optimal control problem given by
\begin{align}
    \min_{\mathbf{U}} \mathcal{J}(\mathbf{U}) & = \min_{\mathbf{U}} \left[ \phi(\mathbf{x}_{T + 1}) + \sum_{t = 1}^{T} \mathcal{L}(\mathbf{x}_t, \mathbf{u}_t) \right] \label{eq/ocp}
,\end{align}
with the initial state $\mathbf{x}_1$ given. Letting the truncated control sequence be $\mathbf{U}_i \defeq \{\mathbf{u}_i, \ldots, \mathbf{u}_T\}$, the value function is given as the cost-to-go starting from a state $\mathbf{x}_i$ and following the optimal control sequence from time $i$ onwards:
\begin{align}
    V(\mathbf{x}_i) & = \min_{\mathbf{U}_i} \left[ \phi(\mathbf{x}_{T + 1}) + \sum_{t = i}^{T} \mathcal{L}(\mathbf{x}_t, \mathbf{u}_t) \right] \label{eq/value_fn}
.\end{align}
Bellman's principle of optimality allows us to rewrite the minimization in \cref{eq/value_fn} recursively as
\begin{align}
    V(\mathbf{x}_i) & = \min_{\mathbf{u}_i} \Big[ \underbrace{\mathcal{L}(\mathbf{x}_i, \mathbf{u}_i) + V(\mathbf{x}_{i + 1})}_{\defeq Q(\mathbf{x}_i, \mathbf{u}_i)} \Big] \label{eq/value_fn_recursive}
,\end{align}
with boundary condition $V(\mathbf{x}_{T + 1}) = \phi(\mathbf{x}_{T + 1})$. \ac{DDP} solves for a quadratic approximation of the value function along a nominal trajectory $\bar{\mathbf{x}}_t$ of the form
\begin{align}
    V(\mathbf{x}_t) & \approx V^0_t + (V^x_t)^\top \delta \mathbf{x}_t + \frac{1}{2} \delta \mathbf{x}_t^\top V^{xx}_t \delta \mathbf{x}_t
,\end{align}
where the superscripts denote the partial derivatives of $V$ evaluated at $\bar{\mathbf{x}}_t$. To solve for the value function derivatives, we consider a quadratic approximation of the $Q$ function defined in \cref{eq/value_fn_recursive} along a nominal state and control trajectory $\bar{\mathbf{x}}_t, \bar{\mathbf{u}}_t$:
\begin{align}
\setlength\arraycolsep{2pt}
    \begin{aligned}
        Q(\mathbf{x}_t, \mathbf{u}_t) \approx {}& Q^0_t + (Q^x_t)^\top \delta \mathbf{x}_t + (Q^u_t)^\top \delta \mathbf{u}_t \\
        & + \frac{1}{2} \begin{bmatrix} \delta \mathbf{x}_t \\ \delta \mathbf{u}_t \end{bmatrix}^\top \begin{bmatrix}
        Q^{xx}_t & (Q^{ux}_t)^\top \\
        Q^{ux}_t & Q^{uu}_t
        \end{bmatrix} \begin{bmatrix} \delta \mathbf{x}_t \\ \delta \mathbf{u}_t \end{bmatrix}
    \end{aligned}
,\end{align}
where
\begin{subequations}
    \begin{align}
        Q^0_t & = \mathcal{L}^0_t + V^0_{t + 1} ,\\
        Q^x_t & = \mathcal{L}^x_t + (\mathbf{F}^x_t)^\top V^x_{t + 1} ,\\
        Q^u_t & = \mathcal{L}^u_t + (\mathbf{F}^u_t)^\top V^x_{t + 1} ,\\
        Q^{xx}_t & = \mathcal{L}^{xx}_t + (\mathbf{F}^x_t)^\top V^{xx}_{t + 1} \mathbf{F}^x_t ,\\
        Q^{ux}_t & = \mathcal{L}^{ux}_t + (\mathbf{F}^u_t)^\top V^{xx}_{t + 1} \mathbf{F}^x_t ,\\
        Q^{uu}_t & = \mathcal{L}^{uu}_t + (\mathbf{F}^u_t)^\top V^{xx}_{t + 1} \mathbf{F}^u_t
    .\end{align} \label{eq/Q_derivatives}
\end{subequations}
Substituting this quadratic approximation into \eqref{eq/value_fn_recursive}, the optimal $\delta \mathbf{u}_t$ is given by
\begin{align}
    \delta \mathbf{u}_t^* & = \argmin_{\delta \mathbf{u}_t} Q(\bar{\mathbf{x}}_t + \delta \mathbf{x}_t, \bar{\mathbf{u}}_t + \delta \mathbf{u}_t) = \mathbf{k}_t + \mathbf{K}_t \delta \mathbf{x}_t \label{eq/optimal_control_update_DDP}
,\end{align}
with
\begin{subequations}
    \begin{align}
        \mathbf{k}_t & \defeq - (Q^{uu}_t)^{-1} Q^u_t ,\\
        \mathbf{K}_t & \defeq - (Q^{uu}_t)^{-1} Q^{ux}_t
    .\end{align}
\end{subequations}
To ensure convergence, the feedforward gain is scaled by a parameter $0 < \epsilon \leq 1$ ensuring that the cost is reduced at every iteration.
Substituting this expression for $\delta \mathbf{u}_t^*$ in to the quadratic expansion of $Q$ and equating like terms with $V$ gives the following expression for the value function derivatives
\begin{subequations}
    \begin{align}
        V^0_t & = Q^0_t - \frac{1}{2} (Q^u_t)^\top (Q^{uu}_t)^{-1} Q^u_t ,\\
        V^x_t & = Q^x_t - (Q^{ux}_t)^\top (Q^{uu}_t)^{-1} Q^u_t ,\\
        V^{xx}_t & = Q^{xx}_t - (Q^{ux}_t)^\top (Q^{uu}_t)^{-1} Q^{ux}_t
    .\end{align} \label{eq/V_derivatives}
\end{subequations}

This gives equations for propagating the value function backwards in time, with boundary conditions $V^0_{T + 1} = \phi^0_{T + 1}$, $V^x_{T + 1} = \phi^x_{T + 1}$, and $V^{xx}_{T + 1} = \phi^{xx}_{T + 1}$. Solving \cref{eq/V_derivatives,eq/Q_derivatives} backwards in time up to the initial condition $\mathbf{x}_1$ constitutes the backward pass of \ac{DDP}.

The forward pass of \ac{DDP} is given by forward simulating the dynamics \eqref{eq/dynamics} starting from $\mathbf{x}_1$ and applying the optimal control update given in \cref{eq/optimal_control_update}. To ensure convergence, the feedforward gain $\mathbf{k}_t$ is scaled by a line search parameter $0 < \epsilon \leq 1$ that is initialized to 1 and iteratively reduced if the cost is not reduced.
\begin{align}
    \delta \mathbf{u}_t^* = \epsilon \mathbf{k}_t + \mathbf{K}_t \delta \mathbf{x}_t
.\end{align}


==> sections/related_work.tex <==
\section{Related Work}
\label{sec/related_work}

Most related to our work is \cite{kobilarov2015differential} and \cite{li2020hybrid}, which use the value function estimates $V_{\mathbf{z}}$ and $V_{\mathbf{zz}}$ to iteratively update the parameters of their respective tasks.

